Power Flow as Intersection of Circles: A new Fixed Point Method

The power flow (PF) problem is a fundamental problem in power system engineering. Many popular solvers face challenges, such as convergence issues. One can try to rewrite the PF problem into a fixed point equation, which can be solved exponentially fast. But, existing methods have their own restrictions, such as the required AC network structure or bus types. To remove these restrictions, we employ the circle geometry per-bus via rectangular coordinate representation to embed our physical knowledge of operation point selection in PV curves. Each iteration of the algorithm consists of finding intersections of circles, which can be computed efficiently with high numerical accuracy. Such analysis also helps in visualizing PV curve to always select the high voltage solution. We compare the performance of our fixed point algorithm with existing state-of-the-art methods, showing that the proposed method can correctly find the solutions when other methods cannot. In addition, we empirically show that the fixed point algorithm is much more robust to bad initialization points than the existing methods.

==> 3bus.tex <==
%% !TEX root=main.tex



\subsection{3-Tuple Representation of Power Flow Equations}
\label{sec:subsec_3tup_rep}








   Comparing \eqref{eq:point_on_a_circle1} and \eqref{eq:point_on_a_circle2} with \eqref{eq:base_form}, the set of points $\mathit{\reallywidebar{\textbf{X}}}$ (roots) in the real Euclidean plane that satisfy the real and reactive power circles are $\mathit{\reallywidebar{\textbf{V}}} = \begin{bmatrix} \mathit{v}_{d,r} &  \mathit{v}_{d,i} \end{bmatrix}^T$.

   From these tuple representation, a real power circle at bus $d$ maybe represented by scalars $\mathit{a}_1$, $\mathit{c}_1$, and a vector $\mathit{\reallywidebar{\textbf{b}}}_1$. Similarly for the reactive power circle as well. The power flow circles are now presented in form of a 3-tuple. It is also important to derive a simple representation of centers and radii of the power flow circles for further calculations. Centers and radii of power flow circles \eqref{eq:cpq}, \eqref{eq:rp} and \eqref{eq:rq} are represented in a simple form by using the elements of their respective 3-tuple representation of power flow circle as shown below
   \begin{align}
   &\mathit{c}_{p} = \dfrac{-\mathit{\reallywidebar{\textbf{b}}}_{1}}{2}, \mathit{c}_{q} = \dfrac{-\mathit{\reallywidebar{\textbf{b}}}_{2}}{2}, \label{eq:cpq_tuple} \\ \notag \\
   &\mathit{r}^2_{p} = \left(\dfrac{\mathit{\reallywidebar{\textbf{b}}}_{1}\cdot \mathit{\reallywidebar{\textbf{b}}}_{1}}{4} - \mathit{c}_{1}\right), \mathit{r}^2_{q} = \left(\dfrac{\mathit{\reallywidebar{\textbf{b}}}_{2}\cdot \mathit{\reallywidebar{\textbf{b}}}_{2}}{4} - \mathit{c}_{2}\right).\label{eq:rpq_tuple}
   \end{align}

		\begin{figure*}[!ht]
	\centering
	\begin{subfigure}{0.375\textwidth}
		\includegraphics[width=\textwidth]{Picture1_3bus.png}
		\caption{P and Q ``circles" at bus 3.}
		\label{fig1}
	\end{subfigure}
	~
	\begin{subfigure}{0.375\textwidth}
		\includegraphics[width=\textwidth]{Picture1_2bus.png}
		\caption{P and Q ``circles" at bus 2.}
		\label{fig2}
	\end{subfigure}
	\caption{Power flow solver  for a  3 bus network.}
	\label{fig:margincomp}
\end{figure*}

The real and reactive power at bus ``d" are represented by \eqref{eq:p_tup} and \eqref{eq:q_tup} respectively. These are further simplified as shown below to obtain the fixed-point equation later in Section~\ref{sec:FPE_powerflow_prob}.

\subsubsection{Real Power Circle Simplification} \eqref{eq:p_tup} is further simplified as shown below.

\begin{align}
\mathit{\reallywidebar{\textbf{b}}}_{1} = \begin{bmatrix}\dfrac{t_{d,2}}{t_{d,1}} \\ \dfrac{t_{d,3}}{t_{d,1}}\end{bmatrix} =\begin{bmatrix}
\dfrac{\sum\limits_{\mathit{k}\in\mathcal{N}(\mathit{d})} (\mathit{v}_{k,r}\mathit{g}_{k,d} - \mathit{v}_{k,i}\mathit{b}_{k,d})}{- \sum\limits_{\mathit{k}\in\mathcal{N}(\mathit{d})} \mathit{g}_{k,d}} \\ \dfrac{\sum\limits_{\mathit{k}\in\mathcal{N}(\mathit{d})} (\mathit{v}_{k,r}\mathit{b}_{k,d} + \mathit{v}_{k,i}\mathit{g}_{k,d})}{- \sum\limits_{\mathit{k}\in\mathcal{N}(\mathit{d})} \mathit{g}_{k,d}}
\end{bmatrix}, \notag \end{align}
\begin{align}
=\begin{bmatrix}
\dfrac{\mathit{\reallywidebar{\textbf{v}}}_{\mathit{k},r} \cdot \mathit{\reallywidebar{\textbf{g}}}_{\mathit{k},d} - \mathit{\reallywidebar{\textbf{v}}}_{\mathit{k},i} \cdot \mathit{\reallywidebar{\textbf{b}}}_{\mathit{k},d}}{- \sum\limits_{i = 1}^{d+1 - \{d\} } \mathit{\reallywidebar{\textbf{g}}(i)}_{k,d}} \\ \dfrac{\mathit{\reallywidebar{\textbf{v}}}_{\mathit{k},r} \cdot \mathit{\reallywidebar{\textbf{b}}}_{\mathit{k},d} + \mathit{\reallywidebar{\textbf{v}}}_{\mathit{k},i} \cdot \mathit{\reallywidebar{\textbf{g}}}_{\mathit{k},d}}{- \sum\limits_{i = 1}^{d+1 - \{d\} } \mathit{\reallywidebar{\textbf{g}}(i)}_{k,d}}
\end{bmatrix} =\begin{bmatrix}
\dfrac{\mathit{\reallywidebar{\textbf{u}}}_{1} \cdot \mathit{\reallywidebar{\textbf{g}}}_{\mathit{k},d} - \mathit{\reallywidebar{\textbf{u}}}_{2} \cdot \mathit{\reallywidebar{\textbf{b}}}_{\mathit{k},d}}{- \sum \mathit{\reallywidebar{\textbf{g}}}_{k,d}} \\ \dfrac{\mathit{\reallywidebar{\textbf{u}}}_{1} \cdot \mathit{\reallywidebar{\textbf{b}}}_{\mathit{k},d} + \mathit{\reallywidebar{\textbf{u}}}_{2} \cdot \mathit{\reallywidebar{\textbf{g}}}_{\mathit{k},d}}{- \sum \mathit{\reallywidebar{\textbf{g}}}_{k,d}}
\end{bmatrix}, \notag \end{align}
\begin{align}
= \dfrac{-1}{\sum \mathit{\reallywidebar{\textbf{g}}}_{k,d}} \cdot
\begin{bmatrix}
\mathit{\reallywidebar{\textbf{g}}}_{k,d} & -\mathit{\reallywidebar{\textbf{b}}}_{k,d} \\ \mathit{\reallywidebar{\textbf{b}}}_{k,d} & \mathit{\reallywidebar{\textbf{g}}}_{k,d}
\end{bmatrix} \cdot
\begin{bmatrix}
\mathit{\reallywidebar{\textbf{u}}}_{1} \\ \mathit{\reallywidebar{\textbf{u}}}_{2}
\end{bmatrix}. \notag
\end{align}
where
%\setlength{\abovedisplayskip}{2pt}
%\setlength{\belowdisplayskip}{2pt}
%\vspace{-1.5cm}
\begin{align}
\mathit{\reallywidebar{\textbf{g}}}_{k,d} &= \begin{bmatrix}\mathit{g}_{1,d} & \mathit{g}_{2,d} & \cdots & \mathit{g}_{d-1,d} & \mathit{g}_{d+1,d}\end{bmatrix}, \notag \\
\mathit{\reallywidebar{\textbf{b}}}_{k,d} &= \begin{bmatrix}\mathit{b}_{1,d} & \mathit{b}_{2,d} & \cdots & \mathit{b}_{d-1,d}& \mathit{b}_{d+1,d}\end{bmatrix}, \notag \\
\mathit{\reallywidebar{\textbf{v}}}_{\mathit{k},r} &= \begin{bmatrix}\mathit{v}_{1,r} & \mathit{v}_{2,r} & \cdots & \mathit{v}_{d-1,r}& \mathit{v}_{d+1,r}\end{bmatrix}^T = \mathit{\reallywidebar{\textbf{u}}}_{1}, \notag \\
\mathit{\reallywidebar{\textbf{v}}}_{\mathit{k},i} &= \begin{bmatrix}\mathit{v}_{1,i} & \mathit{v}_{2,i} & \cdots & \mathit{v}_{d-1,i} & \mathit{v}_{d+1,i}~ \end{bmatrix}^T = \mathit{\reallywidebar{\textbf{u}}}_{2}, \notag
\end{align}
buses 1, 2, $\cdots$, $d-1$ and $d+1$ are the neighboring buses to bus $d$.

Let $\mathit{\reallywidebar{\textbf{U}}}$ represents the neighboring voltages of bus ``d" then $\mathit{\reallywidebar{\textbf{U}}} = \begin{bmatrix} \mathit{\reallywidebar{\textbf{u}}}_{1} \\ \mathit{\reallywidebar{\textbf{u}}}_{2} \end{bmatrix}$. Let us define few constants for ease of representation, where
\begin{align}
\alpha &= \dfrac{\mathit{\reallywidebar{\textbf{g}}}_{k,d}}{\sum\mathit{\reallywidebar{\textbf{g}}}_{k,d}}, \beta = \dfrac{\mathit{\reallywidebar{\textbf{b}}}_{k,d}}{\sum\mathit{\reallywidebar{\textbf{b}}}_{k,d}}, \notag \\ \notag \\
\gamma &= \dfrac{\mathit{\reallywidebar{\textbf{g}}}_{k,d}}{\sum\mathit{\reallywidebar{\textbf{b}}}_{k,d}}, \delta = \dfrac{\mathit{\reallywidebar{\textbf{b}}}_{k,d}}{\sum\mathit{\reallywidebar{\textbf{g}}}_{k,d}}. \notag
\end{align}

The simplified 3-tuple representation of the real power circle is
 \begin{align} &= \left\lbrace 1, 	\dfrac{-1}{\sum \mathit{\reallywidebar{\textbf{g}}}_{k,d}} \cdot
\begin{bmatrix}
\mathit{\reallywidebar{\textbf{g}}}_{k,d} & -\mathit{\reallywidebar{\textbf{b}}}_{k,d} \\ \mathit{\reallywidebar{\textbf{b}}}_{k,d} & \mathit{\reallywidebar{\textbf{g}}}_{k,d}
\end{bmatrix} \cdot \mathit{\reallywidebar{\textbf{U}}},\dfrac{\mathit{p}_{d}}{\sum \mathit{\reallywidebar{\textbf{g}}}_{k,d}} \right \rbrace, \notag \\ \notag \\
 &= \left\lbrace 1,
 \begin{bmatrix}
-\alpha & \delta \\ -\delta & -\alpha
\end{bmatrix} \cdot \mathit{\reallywidebar{\textbf{U}}},\dfrac{\mathit{p}_{d}}{\sum \mathit{\reallywidebar{\textbf{g}}}_{k,d}} \right \rbrace. \label{eq:3tuple_P} \end{align}

\subsubsection{Reactive Power Circle Simplification} \eqref{eq:q_tup} is further simplified as shown below.

\begin{align}
\mathit{\reallywidebar{\textbf{b}}}_{2} &= \begin{bmatrix}\dfrac{-t_{d,3}}{t_{d,4}} \\ \dfrac{t_{d,2}}{t_{d,4}}\end{bmatrix}
=\begin{bmatrix}
\dfrac{-\sum\limits_{\mathit{k}\in\mathcal{N}(\mathit{d})} (\mathit{v}_{k,r}\mathit{b}_{k,d} + \mathit{v}_{k,i}\mathit{g}_{k,d})}{\sum\limits_{\mathit{k}\in\mathcal{N}(\mathit{d})} \mathit{b}_{k,d}} \\ \dfrac{\sum\limits_{\mathit{k}\in\mathcal{N}(\mathit{d})} (\mathit{v}_{k,r}\mathit{g}_{k,d} - \mathit{v}_{k,i}\mathit{b}_{k,d})}{\sum\limits_{\mathit{k}\in\mathcal{N}(\mathit{d})} \mathit{b}_{k,d}}
\end{bmatrix},\notag \end{align}
\begin{align}
&=\begin{bmatrix}
\dfrac{-(\mathit{\reallywidebar{\textbf{v}}}_{\mathit{k},r} \cdot \mathit{\reallywidebar{\textbf{b}}}_{\mathit{k},d} + \mathit{\reallywidebar{\textbf{v}}}_{\mathit{k},i} \cdot \mathit{\reallywidebar{\textbf{g}}}_{\mathit{k},d})}{\sum\limits_{i = 1}^{d+1 - \{d\}} \mathit{\reallywidebar{\textbf{b}}(i)}_{k,d}} \\ \dfrac{\mathit{\reallywidebar{\textbf{v}}}_{\mathit{k},r} \cdot \mathit{\reallywidebar{\textbf{g}}}_{\mathit{k},d} - \mathit{\reallywidebar{\textbf{v}}}_{\mathit{k},i} \cdot \mathit{\reallywidebar{\textbf{b}}}_{\mathit{k},d}}{\sum\limits_{i = 1}^{d+1 - \{d\}} \mathit{\reallywidebar{\textbf{b}}(i)}_{k,d}}
\end{bmatrix} =\begin{bmatrix}
\dfrac{-(\mathit{\reallywidebar{\textbf{u}}}_{1} \cdot \mathit{\reallywidebar{\textbf{b}}}_{\mathit{k},d} + \mathit{\reallywidebar{\textbf{u}}}_{2} \cdot \mathit{\reallywidebar{\textbf{g}}}_{\mathit{k},d})}{\sum \mathit{\reallywidebar{\textbf{b}}}_{k,d}} \\ \dfrac{\mathit{\reallywidebar{\textbf{u}}}_{1} \cdot \mathit{\reallywidebar{\textbf{g}}}_{\mathit{k},d} - \mathit{\reallywidebar{\textbf{u}}}_{2} \cdot \mathit{\reallywidebar{\textbf{b}}}_{\mathit{k},d}}{\sum \mathit{\reallywidebar{\textbf{b}}}_{k,d}}
\end{bmatrix},\notag \end{align}
\begin{align}
&= \dfrac{1}{\sum \mathit{\reallywidebar{\textbf{b}}}_{k,d}} \cdot
\begin{bmatrix}
-\mathit{\reallywidebar{\textbf{b}}}_{k,d} & -\mathit{\reallywidebar{\textbf{g}}}_{k,d} \\ \mathit{\reallywidebar{\textbf{g}}}_{k,d} & -\mathit{\reallywidebar{\textbf{b}}}_{k,d}
\end{bmatrix} \cdot
\begin{bmatrix}
\mathit{\reallywidebar{\textbf{u}}}_{1} \\ \mathit{\reallywidebar{\textbf{u}}}_{2}
\end{bmatrix}. \notag
\end{align}

The simplified 3-tuple representation of the reactive power circle is

\begin{align} &=\left\lbrace 1, 	\dfrac{1}{\sum \mathit{\reallywidebar{\textbf{b}}}_{k,d}} \cdot
\begin{bmatrix}
-\mathit{\reallywidebar{\textbf{b}}}_{k,d} & -\mathit{\reallywidebar{\textbf{g}}}_{k,d} \\ \mathit{\reallywidebar{\textbf{g}}}_{k,d} & -\mathit{\reallywidebar{\textbf{b}}}_{k,d}
\end{bmatrix} \cdot \mathit{\reallywidebar{\textbf{U}}},\dfrac{-\mathit{q}_{d}}{\sum \mathit{\reallywidebar{\textbf{b}}}_{k,d}} \right \rbrace, \notag \\ \notag \\
 &= \left\lbrace 1,
\begin{bmatrix}
-\beta & -\gamma \\ \gamma & -\beta
\end{bmatrix} \cdot \mathit{\reallywidebar{\textbf{U}}},\dfrac{\mathit{p}_{d}}{\sum \mathit{\reallywidebar{\textbf{g}}}_{k,d}} \right \rbrace. \label{eq:3tuple_Q}
 \end{align}

